Automated Expected Amortised Cost Analysis of Probabilistic Data Structures

In this paper, we present the first fully-automated expected amortised cost analysis of self-adjusting data structures, that is, of randomised splay trees, randomised splay heaps and randomised meldable heaps, which so far have only (semi-) manually been analysed in the literature. Our analysis is stated as a type-and-effect system for a first-order functional programming language with support for sampling over discrete distributions, non-deterministic choice and a ticking operator. The latter allows for the specification of fine-grained cost models. We state two soundness theorems based on two different -- but strongly related -- typing rules of ticking, which account differently for the cost of non-terminating computations. Finally we provide a prototype implementation able to fully automatically analyse the aforementioned case studies.

==> rules/sem/appA.tex <==
\infer
  {\evalkn{\sigma}{\kappa}{n+1}{c}{f~x_1~\dots~x_k}{\mu}}
  {f~y_1~\dots~y_k \flst{ = } e \in \Program & \evalkn{\sigma'}{\kappa}{n}{c}{e}{\mu}}


==> rules/sem/cmp.tex <==
\infer
  {\evaln{\sigma}{0}{0}{x_1 \circ x_2}{b}}
  {\text{$b$ is value of $x_1\sigma \circ x_2\sigma$}}


==> rules/sem/coinA.tex <==
\infer
  {\evalkn{\sigma}{\kappa}{n+1}{pc_1 + (1-p)c_2}{\flstk{if } \coin[$a$][$b$] \flstk{ then }e_1\flstk{ else }e_2}{p\mu_1+(1-p)\mu_2}}
  {\evalkn{\sigma}{\kappa}{n}{c_1}{e_1}{\mu_1} & \evalkn{\sigma}{\kappa}{n}{c_2}{e_2}{\mu_2} & p = \sfrac{a}{b}}


==> rules/sem/false.tex <==
\infer{\eval{\sigma}{0}{\flstc{false}}{\flstc{false}}}{}


==> rules/sem/itefalseA.tex <==
\infer
  {\evalkn{\sigma}{\kappa}{n+1}{c}{\flstk{if }x\flstk{ then }e_1\flstk{ else }e_2}{\mu}}
  {x\sigma = \flstk{false} & \evalkn{\sigma}{\kappa}{n}{c}{e_2}{\mu}}


==> rules/sem/itetrueA.tex <==
\infer
  {\evalkn{\sigma}{\kappa}{n+1}{c}{\flstk{if }x\flstk{ then }e_1\flstk{ else }e_2}{\mu}}
  {x\sigma=\flstk{true} & \evalkn{\sigma}{\kappa}{n}{c}{e_1}{\mu}}


==> rules/sem/leafA.tex <==
\infer{\evalkn{\sigma}{\kappa}{0}{\kappa}{\flstc{leaf}}{\{\flstc{leaf}^1\}}}{}


==> rules/sem/letA.tex <==
% \infer{\evalkn{\sigma}{\kappa}{n+1}{\sum_{w \in \supp{\nu}} \nu(w) \cdot c_w}{\flstk{let }x\flst{ = }e_1\flstk{ in }e_2}{\sum_{w \in \supp{\nu}} \nu(w) \cdot \mu_w}}%
%   {%
%   \evalkn{\sigma}{0}{n}{c_1}{e_1}{\nu}
%   &
%   \text{for all $w \in \supp{\nu}$:
%   $\evalkn{\sigma[x \mapsto w]}{\kappa+ (\nu(w)\cdot c_1)}{n}{c_w}{e_2}{\mu_w}$
%   }
%   }
% GM: overapproximation
\infer{\evalkn{\sigma}{\kappa}{n+1}{\sum_{w \in \supp{\nu}} \nu(w) \cdot c_w}{\flstk{let }x\flst{ = }e_1\flstk{ in }e_2}{\sum_{w \in \supp{\nu}} \nu(w) \cdot \mu_w}}%
  {%
  \evalkn{\sigma}{0}{n}{c_1}{e_1}{\nu}
  &
  \text{for all $w \in \supp{\nu}$:
  $\evalkn{\sigma[x \mapsto w]}{\kappa+c_1}{n}{c_w}{e_2}{\mu_w}$
  }
  }


==> rules/sem/matchleafA.tex <==
\infer
  {\evalkn{\sigma}{\kappa}{n+1}{c}{\flstk{match }x\flstk{ with} \begin{array}[t]{l}%
    \flst{| } \flstc{leaf} \flst{ -> } e_1 \\
    \flst{| } \text{\flsttree{$x_0$}{$x_1$}{$x_2$}} \flst{ -> } e_2
  \end{array}}{\mu}}
  {x\sigma = \flstc{leaf} & \evalkn{\sigma}{\kappa}{n}{c}{e_1}{\mu}}


==> rules/sem/matchnodeA.tex <==
\infer
  {\evalkn{\sigma}{\kappa}{n+1}{c}{\flstk{match }x\flstk{ with} \begin{array}[t]{l}%
    \flst{| } \flstc{leaf} \flst{ -> }e_1 \\
    \flst{| } \text{\flsttree{$x_0$}{$x_1$}{$x_2$}} \flst{ -> } e_2
  \end{array}}{\mu}}
  {x\sigma = \text{\flsttree{$t$}{$a$}{$u$}} & \evalkn{\sigma''}{\kappa}{n}{c}{e_2}{\mu}}


==> rules/sem/matchpairA.tex <==
\infer
  {\evalkn{\sigma}{\kappa}{n+1}{c}{\flstk{match }x\flstk{ with} \begin{array}[t]{l}%
    \flst{| } \text{\flstpair{$x_1$}{$x_2$}} \flst{ -> } e \\
  \end{array}}{\mu}}
  {x\sigma = \text{\flstpair{$t$}{$u$}} & \evalkn{\sigma'''}{\kappa}{n}{c}{e}{\mu}}


==> rules/sem/nodeA.tex <==
\infer{\evalkn{\sigma}{\kappa}{0}{\kappa}{\text{\flsttree{$x_1$}{$x_2$}{$x_3$}}}{\{(\text{\flsttree{$t$}{$b$}{$u$}})^1\}}}%
  {x_1\sigma = t
  &x_2\sigma = b
  &x_3\sigma = u} 


==> rules/sem/nonvalA.tex <==
\infer
  {\evalkn{\sigma}{\kappa}{0}{0}{e}{\{\}}}
  {e \text{ is not a value}}


==> rules/sem/pairA.tex <==
\infer{\evalkn{\sigma}{\kappa}{0}{\kappa}{\text{\flstpair{$x_1$}{$x_2$}}}{\{{\text{\flstpair{$t$}{$u$}}}^1\}}}%
{x_1\sigma = t
  &
  x_2\sigma = u
}

==> rules/sem/tick.tex <==
% NOTE(lorenz): Why can we not use x_1~\dots~x_n ? Is n used for anything?
% GM tick in LNF
% \infer{%
% \evaln{\sigma}{0}{\sfrac{a}{b}}{\tick[$a$][$b$]}{\{\tick[$a$][$b$]^1\}}
% }{}
% GM: ticking as function
\infer
  {\evaln{\sigma}{n+1}{c+\sfrac{a}{b}}{\tick[$a$][$b$]{e}}{\mu}}
  {\evaln{\sigma}{n}{c}{e}{\mu}}

==> rules/sem/tickA.tex <==
\infer
  {\evalkn{\sigma}{\kappa}{n+1}{c}{\tick[$a$][$b$]{e}}{\tick[$a$][$b$]{\mu}}}
  {\evalkn{\sigma}{\kappa+\sfrac{a}{b}}{n}{c}{e}{\mu}}

==> rules/sem/true.tex <==
\infer{\eval{\sigma}{0}{\flstc{true}}{\flstc{true}}}{}


==> rules/sem/varA.tex <==
\infer{\evalkn{\sigma}{\kappa}{0}{\kappa}{x}{\{v^1\}}}{x\sigma = v}


==> rules/typ/letgen.tex <==
% \infer[\ruleletgen]{
%   \tjudge{\Gamma, \Delta}{Q}{\flstk{let }x\flst{ = }e_1\flstk{ in }e_2}{\beta}{Q'}
% }{%
%   \begin{minipage}[b]{25ex}
%     % $p_i = q_i \quad p_{(\veca,c)} = q_{(\veca, \vec{0}, c)}$\\[2ex]
%     % $\tjudge{\Gamma}{P}{e_1}{\alpha}{P'}$
%     $p_i = q_i \quad p_{(\veca,c)} = q_{(\veca, \vec{0}, c)}$\\[2ex]
%     $\tjudge{\Gamma}{P}{e_1}{\alpha}{P'}$
%   \end{minipage}
%   &
%   \begin{minipage}[b]{25ex}
%     $\forall \vec{b} \not= \vec{0} \left( q_{(\vec{0},\vec{b},c)} = r_{(\vec{b},c)} \right)$ \\[2ex]
%     $\tjudge{\Delta, \typed{x}{\alpha}}{R}{e_2}{\beta}{Q'}$
%   \end{minipage}
%   &
%   \begin{minipage}[b]{25ex}
%     $r_{(\vec{0},c)} = p'_{(c)} \quad r_j = q_{m+j}$\\[2ex]
%     $\alpha \not= \TreeShort$
%   \end{minipage}
% }
% GM new version for trees and non-trees
\infer[\ruleletgen]{
  \tjudge{\Gamma, \Delta}{Q}{\flstk{let }x\flst{ = }e_1\flstk{ in }e_2}{\beta}{Q'}
}{%
  \begin{minipage}[b]{25ex}
    $p_i = q_i \quad p_{(\veca,c)} = q_{(\veca, \vec{0}, c)}$\\[2ex]
    $\tjudge{\Gamma}{P}{e_1}{\alpha}{P'}$
  \end{minipage}
  &
  \begin{minipage}[b]{27ex}
    $\forall \vec{b} \not= \vec{0} \left( q_{(\vec{0},\vec{b},c)} = r_{(\vec{b},0,c)} \right)$ \\[2ex]
    $\tjudge{\Delta, \typed{x}{\alpha}}{R}{e_2}{\beta}{Q'}$
  \end{minipage}
  &
  \begin{minipage}[b]{25ex}
    $r_{(\vec{0},a,c)} = p'_{(a,c)} 
    \\[2ex]
    r_{k+1} = p'_{*} \quad r_{k+1} = p'_{\ast}$ %    $\alpha \not= \TreeShort$
  \end{minipage}
}

